Productive Multitasking for Industrial Robots

The application of robotic solutions to small-batch production is challenging: economical constraints tend to dramatically limit the time for setting up new batches. Organizing robot tasks into modular software components, called skills, and allowing the assignment of multiple concurrent tasks to a single robot is potentially game-changing. However, due to cycle time constraints, it may be necessary for a skill to take over without waiting on another to terminate, and the available literature lacks a systematic approach in this case. In the present article, we fill the gap by (a) establishing the specifications of skills that can be sequenced with partial executions, (b) proposing an implementation based on the combination of finite-state machines and behavior trees, and (c) demonstrating the benefits of such skills through extensive trials in the environment of ARIAC (Agile Robotics for Industrial Automation Competition).

==> tex/application.tex <==

\section{Application}
\label{sec:application}

\begin{figure}[t]
    \centering
    \vspace{3mm}
    \includegraphics[width = 0.5 \columnwidth]{jpg/experiment.jpg}
    \caption{Experimental setup for the application of our approach on the operation of picking up a piston with a pneumatic gripper.
    }
    \label{fig:setup}
\end{figure}

We applied our approach to the operation of picking up a piston with a pneumatic gripper.
Fig.\ref{fig:setup} shows our experimental setup.
This operation fits in the industrial use-case of Fig.~\ref{fig:cobot},
where this piston has to be assembled on an engine block.
In particular, we designed a pickup skill that can be preempted at anytime by a place skill
in order to restore the work-space in its initial configuration.
Figure~\ref{fig:ssm} gives the corresponding SSM,
featuring switches of control modes and detection of contact forces.
The transitions associated with "pickup" define the usual execution,
while the ones associated with "place" allow to reverse this execution at any time.
Note the presence of a second edge associated with the pickup skill on the "reach" node:
it allows to deal with the case where the piston is missing.
The accompagning video illustrate the experiment we conducted on this setup.

\begin{figure}[t]
    \centering
    \includegraphics[width = 0.9 \columnwidth]{pdf/ssm.pdf}
    \caption{The skill state machine designed for the application of our approach.
    Otherwise mentioned, every condition consist of positional tolerances.
    The skill identifiers in the nodes denote terminations,
    and the exclamation points on the edges, imperative conditions.}
    \label{fig:ssm}
\end{figure}


==> tex/conclusion.tex <==

\section{Conclusion}
\label{sec:conclusion}

% We explored the possibility of assigning multiple tasks to a single robot
% when the presence of time constraints enforces switches between tasks.
% Assuming the availability of an adequate robot controller,
% our approach supports instantaneous reactions to changes of context at the lowest level---analogously to \textit{reflexes}.
% Our experimentation in ARIAC demonstrated the benefit of preemptive skills.
% Future works could include a quantitative assessment of the benefits of combining BTs and FSMs
% using complexity metrics.

% -We noted that we need both BTs and HFSMs for ARIAC
% -We proposed in this paper a framework for a systematic implementation of preemptive skills
% -We demonstrate the use of the framework in the ARIAC competition and show the benefit of preemptive skills w.r.t. non-preemptive ones.

Inspired by the many challenges raised in ARIAC,
we explored the possibility of assigning multiple tasks to an industrial robot
with time constraints enforcing fast switching between tasks.
We identified the need for a notion of preemption related to the execution of robot skills,
Like the BTs before, the BT-FSM model that we introduced here was also motivated by know-how from the video gaming industry.
We demonstrated the use of this framework in the environment of ARIAC
and showed the benefits of preemptive skills w.r.t. non-preemptive ones.
Our implementation resulted in a robot capable of reacting instantaneously
to the occurrences of non-deterministic events\textemdash
similarly to \textit{reflexes}, but without short-circuiting any deliberative loop.
Future works could include the application of complexity metrics to BTS and FSMs
in order to determine in which cases one model is preferable over the other.

\section*{Acknowledgment}

The authors would like to thank the National Institute of Standards and Technology (NIST)
and the Open Source Robotics Foundation (OSRF)
for organizing the Agile Robotics for Industrial Automation Competition (ARIAC).


==> tex/draft.tex <==

\section*{Draft}

%\dw{
%  \begin{itemize}
 %   \item Introduce the mass-customization context
  %  \item Introduce the skill-based programming approach
   % \item Introduce industrial robotic tasks
    %\item Define:
     % \begin{itemize}
      %  \item Task:
       % \item Skill:
        %\item Primitive:
%      \end{itemize}
 %   \item Introduce the need for reactivity in task execution
  %  \item Define reactivity in task execution
   % \item Define the possible reactions that can be expected during task execution:
   % \begin{itemize}
    %  \item Emergency stop:
     % \item Preemption:
      %\item Reversion:
      %\item New task:
%    \end{itemize}
 %   \item Explain how preemption turns out to be the simplest way to introduce reactivity in task execution
  %  \item Layout specifications for preemptable task execution
   % \item Try with FSM (Finite State-Machines):
    %  \begin{itemize}
     %   \item Give the formal definition of FSM
      %  \item Give the general mechanism for implementing preemption with FSMs
%        \item Give a toy-example
 %       \item Discuss the pros and cons
  %      \item Try to reach the conclusion that FSMs are good for capturing the structure of industrial robotic tasks,
   %       but bad in terms of reactivity
    %  \end{itemize}
    %\item Try with BTs (Behavior Trees):
     % \begin{itemize}
      %  \item Give the formal definition of BTs
       % \item Give the general mechanism for implementing preemption with BTs
       % \item Remix the toy-example
    %    \item Discuss the pros and cons
     %   \item Try to reach the conclusion that behavior trees are good in terms of reactivity,
     %     but bad in terms of capturing the structure of industrial robotic tasks
     % \end{itemize}
    %\item Propose to unify FSMs and BTs in a novel low-level coordination mechanism
%    \item Argue that BTs are already relying on FSMs on their leaf nodes
 %   \item Give its formal definition
  %  \item Explain how it deals with preemption
  %  \item Remix the toy-example
   % \item Discuss the pros and cons
%    \item Try to reach the conclusion that it gets the bests out of FSMs and BTs in the context of industrial robotic tasks
 % \end{itemize}
%}



==> tex/results.tex <==

\section{Evaluation}
\label{sec:results}

\begin{figure}[t]
\centering
\includegraphics[width = 0.95 \columnwidth]{pdf/result.pdf}
\caption{Results.}
\label{fig:result}
\end{figure}

